Genetic Algorithms For Parameter Optimization for Disparity Map Generation of Radiata Pine Branch Images

Traditional stereo matching algorithms like Semi-Global Block Matching (SGBM) with Weighted Least Squares (WLS) filtering offer speed advantages over neural networks for UAV applications, generating disparity maps in approximately 0.5 seconds per frame. However, these algorithms require meticulous parameter tuning. We propose a Genetic Algorithm (GA) based parameter optimization framework that systematically searches for optimal parameter configurations for SGBM and WLS, enabling UAVs to measure distances to tree branches with enhanced precision while maintaining processing efficiency. Our contributions include: (1) a novel GA-based parameter optimization framework that eliminates manual tuning; (2) a comprehensive evaluation methodology using multiple image quality metrics; and (3) a practical solution for resource-constrained UAV systems. Experimental results demonstrate that our GA-optimized approach reduces Mean Squared Error by 42.86% while increasing Peak Signal-to-Noise Ratio and Structural Similarity by 8.47% and 28.52%, respectively, compared with baseline configurations. Furthermore, our approach demonstrates superior generalization performance across varied imaging conditions, which is critcal for real-world forestry applications.

==> ideal.tex <==
%\documentclass[conference]{IEEEtran}
%\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
%Template version as of 6/27/2024
% Add the following code after the \maketitle command:

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{url}
\usepackage{booktabs}
\usepackage{subfigure} 
\usepackage{hyperref}

\begin{document}
Benny(Yida Lin)

\section{2025 goal: Deployment on Drone}
In our first year of research, we conducted extensive testing and validation on computers. Therefore, in the second year, I want to apply the algorithms we previously developed to drones and conduct tests on them. If we only continue testing on our own computers, the project will remain in the testing phase indefinitely.




\section{Instance Segmentation}
\section{Optimaization SGBM Paramteres}
\section{Combining Monocular and Stereo Depth Estimation}










%\bibliographystyle{IEEEtran} % 引用樣式文件
%\bibliography{references} % 引用的文獻文件


\vspace{12pt}

\end{document}
